Provable Regret Bounds for Deep Online Learning and Control

The theory of deep learning focuses almost exclusively on supervised learning, non-convex optimization using stochastic gradient descent, and overparametrized neural networks. It is common belief that the optimizer dynamics, network architecture, initialization procedure, and other factors tie together and are all components of its success. This presents theoretical challenges for analyzing state-based and/or online deep learning. Motivated by applications in control, we give a general black-box reduction from deep learning to online convex optimization. This allows us to decouple optimization, regret, expressiveness, and derive agnostic online learning guarantees for fully-connected deep neural networks with ReLU activations. We quantify convergence and regret guarantees for any range of parameters and allow any optimization procedure, such as adaptive gradient methods and second order methods. As an application, we derive provable algorithms for deep control in the online episodic setting.

==> preamble/header-colt.tex <==
\usepackage{float}
\usepackage{algorithm}

\newcommand{\softmax}{\text{softmax}}
\newcommand{\CH}{\text{CH}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\M}{\mathcal{M}}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}
\newcommand{\elad}[1]{$\ll$\textsf{\color{blue} Elad : #1}$\gg$}


\newcommand{\jnote}[1]{$\ll$\textsf{\color{blue} JL : #1}$\gg$}

\def\ltil{{{\tilde{\ell}}}}
\def\btalpha{{\bm{\tilde{\alpha}}}}
\def\balpha{{\bm{\alpha}}}
\def\talpha{{\tilde{\alpha}}}
\def\btbeta{{\bm{\tilde{\beta}}}}
\def\bbeta{{\bm{\beta}}}
\def\tbeta{{\tilde{\beta}}}
\def\btgamma{{\bm{\tilde{\gamma}}}}
\def\bgamma{{\bm{\gamma}}}
\def\tgamma{{\tilde{\gamma}}}


\def\mL{{\mathcal L}}

\def\X{{\mathcal X}}
\def\H{{\mathcal H}}
\def\Y{{\mathcal Y}}
\def\W{{\mathcal W}}
\def\R{{\mathbb R}}
\def\N{{\mathcal N}}

\numberwithin{equation}{section}

% notation here
\newcommand{\ftil}{\tilde{f}}

\def\hestinv{\tilde{\nabla}^{-2}}
\def\hest{\tilde{\nabla}^{2}}
\def\hessinv{\nabla^{-2}}
\def\hess{\nabla^2}
\def\grad{\nabla}


% notation

\newcommand{\re}{{\text{Re}}}
\newcommand{\B}{B}
%\newcommand{\R}{\mathcal{R}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\cE}{\mathcal{E}}
\renewcommand{\sp}{\mathrm{span}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\cor}{\mathrm{cor}}
\newcommand{\sign}{\text{ } \mathrm{sign}}


\newcommand{\bzero}{\ensuremath{\mathbf 0}}
\newcommand{\y}{\ensuremath{\mathbf y}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\h}{\ensuremath{\mathbf h}}
\newcommand{\K}{\ensuremath{\mathcal K}}
\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\C{{\mathcal C}}

%\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
%\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\x{\mathbf{x}}
\def\y{\mathbf{y}}
\def\w{\mathbf{w}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
%\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bS{\mathbf{S}}
\def\bG{\mathbf{G}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}
\def\sysid{\text{SysId}}
\def\frelu{\sigma_{\text{relu}}}

\def\regret{\mbox{{Regret}}}
\def\relu{\mbox{{ReLU }}}
\def\sphere{\mathbb{S}}
\def\ytil{\tilde{{y}}}
\def\yhat{\hat{{y}}}
\def\what{\hat{{w}}}
\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}

\newcommand{\tstart}[1]{s_{#1}}
\newcommand{\tend}[1]{e_{#1}}
\DeclareMathOperator{\OPT}{OPT}
\DeclareMathOperator{\CR}{\mathcal{C}}



% comments, etc
\newcommand{\ignore}[1]{}
\newcommand{\eh}[1]{\noindent{\textcolor{blue}{\{{\bf EH:} \em #1\}}}}
\newcommand{\ug}[1]{\noindent{\textcolor{purple}{\{{\bf UG:} \em #1\}}}}
\newcommand{\xc}[1]{\noindent{\textcolor{orange}{\{{\bf XC:} \em #1\}}}}
\newcommand{\edgar}[1]{\noindent{\textcolor{magenta}{\{{\bf EM:} \em #1\}}}}
% for emails
\newcommand{\email}[1]{\texttt{#1}}

%% JMLR theorems adjustments
%\setlength{\topsep}{\medskipamount}
%
%\newtheoremstyle{jmlrthm} % name
%	{\topsep}		% Space above
%	{\topsep}		% Space below
%	{\itshape}	% Body font
%	{}						% Indent amount
%	{\bfseries}	% Theorem head font
%	{}						% Punctuation after theorem head
%	{0.33em}		% Space after theorem head
%	{}  					% Theorem head spec (can be left empty, meaning ?normal?)
%
%\newtheoremstyle{jmlrdef} % name
%	{\topsep}		% Space above
%	{\topsep}		% Space below
%	{}						% Body font
%	{}						% Indent amount
%	{\bfseries}	% Theorem head font
%	{}						% Punctuation after theorem head
%	{.33em}			% Space after theorem head
%	{}  					% Theorem head spec (can be left empty, meaning ?normal?)
%
%\renewcommand\qedsymbol{\BlackBox}
%%\renewenvironment{proof}[1][Proof]{\par\noindent{\bfseries\upshape #1\ }}{\hfill\BlackBox\\[\medskipamount]}
%\renewenvironment{proof}[1][Proof]{\par\noindent{\bfseries\upshape #1\ }}{\hfill\BlackBox\\}


% theorems
% \theoremstyle{plain}
% % \theoremstyle{jmlrthm}
% % \newtheorem{theorem}{Theorem}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}[lemma]{Proposition}
% \newtheorem{claim}[lemma]{Claim}
% \newtheorem{fact}[lemma]{Fact}
% \newtheorem{observation}[corollary]{Observation}
\newtheorem{assumption}{Assumption}
% \newtheorem{definition}{Definition}[section]

% \newtheorem*{theorem*}{Theorem}
% \newtheorem*{lemma*}{Lemma}
% \newtheorem*{corollary*}{Corollary}
% \newtheorem*{proposition*}{Proposition}
% \newtheorem*{claim*}{Claim}
% \newtheorem*{fact*}{Fact}
% \newtheorem*{observation*}{Observation}
% \newtheorem*{assumption*}{Assumption}

% \theoremstyle{definition}
% %\theoremstyle{jmlrdef}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{example}[theorem]{Example}
% \newtheorem*{definition*}{Definition}
% \newtheorem*{remark*}{Remark}
% \newtheorem*{example*}{Example}


% repeated theorems
%  \theoremstyle{plain}

% \newenvironment{repthm}[2][]{%
%   \def\theoremauxref{\cref{#2}}
%   \begin{theoremaux}[#1]
% }{%
%   \end{theoremaux}
% }

%\newtheoremstyle{theoremrep}
%	{\topsep}{\topsep}              %%% space between body and thm
%	{\itshape}                      %%% Thm body font
%	{}                              %%% Indent amount (empty = no indent)
%	{\bfseries}                     %%% Thm head font
%	{}                             %%% Punctuation after thm head
%	{0.33em}                             %%% Space after thm head
%	{\cref{#3}}
%
%\theoremstyle{theoremrep}
%\newtheorem{repthm}{dontcare}



% % old refs - use \cref{} instead!
% \newcommand{\secref}[1]{Section~\ref{#1}}
%\newcommand{\secref}[1]{Sec.~\ref{#1}}
%\newcommand{\figref}[1]{Figure~\ref{#1}}
%\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
%\newcommand{\lemref}[1]{Lemma~\ref{#1}}

% \newcommand{\thmref}[1]{Theorem~\ref{#1}}
% \newcommand{\appref}[1]{Appendix~\ref{#1}}
% \newcommand{\algref}[1]{Algorithm~\ref{#1}}

% style defs
%\renewcommand{\le}{\leqslant}
%\renewcommand{\ge}{\geqslant}
%\renewcommand{\leq}{\le}
%\renewcommand{\geq}{\ge}

% bold serif
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}

% operators
\DeclareMathOperator*{\err}{error}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\supp}{supp}
%\DeclareMathOperator*{\poly}{poly}
\let\Pr\relax
\DeclareMathOperator{\Pr}{\mathbb{P}}

% cases
\newcommand{\mycases}[4]{{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}}
\end{array}
\right. }}

\newcommand{\mythreecases}[6] {{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}} \\[1ex]
    {#5} & {\;\text{#6}}
\end{array}
\right. }}

% macros
\newcommand{\lr}[1]{\!\left(#1\right)\!}
\newcommand{\lrbig}[1]{\big(#1\big)}
\newcommand{\lrBig}[1]{\Big(#1\Big)}
\newcommand{\lrbra}[1]{\!\left[#1\right]\!}
\newcommand{\lrnorm}[1]{\left\|#1\right\|}
\newcommand{\lrset}[1]{\left\{#1\right\}}
\newcommand{\lrabs}[1]{\left|#1\right|}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\renewcommand{\t}[1]{\smash{\tilde{#1}}}
\newcommand{\wt}[1]{\smash{\widetilde{#1}}}
\newcommand{\wh}[1]{\smash{\widehat{#1}}}
\renewcommand{\O}{O}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\OO}[1]{\O\lr{#1}}
\newcommand{\tO}{\wt{\O}}
\newcommand{\tTheta}{\wt{\Theta}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\lrbra{#1}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\tsum}{\sum\nolimits}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\ind}[1]{\mathbb{I}\!\lrset{#1}}
\newcommand{\non}{\nonumber}
\newcommand{\poly}{\mathrm{poly}}

% \newcommand{\tr}{^{\mathsmaller\top}}
\newcommand{\tr}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\st}{\star}
\renewcommand{\dag}{\dagger}

%\newcommand{\kl}[2]{\mathsf{D}_\mathrm{KL}(#1,#2)}
\newcommand{\tv}[2]{\mathsf{D}_{\mathrm{TV}}(#1,#2)}
\newcommand{\ent}{\mathsf{H}}
\newcommand{\info}{\mathsf{I}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ep}{\varepsilon}
%\newcommand{\eps}{\epsilon}
\newcommand{\sig}{\sigma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\lam}{\lambda}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}

\newcommand{\eqdef}{:=}
\newcommand{\eq}{~=~}
\renewcommand{\leq}{~\le~}
\renewcommand{\geq}{~\ge~}
\newcommand{\lt}{~<~}
\newcommand{\gt}{~>~}
\newcommand{\then}{\quad\Rightarrow\quad}

\let\oldtfrac\tfrac
\renewcommand{\tfrac}[2]{\smash{\oldtfrac{#1}{#2}}}


\let\nablaold\nabla
\renewcommand{\nabla}{\nablaold\mkern-2.5mu}
%\let\cdotold\cdot
%\renewcommand{\cdot}{\mkern-2.5mu\cdotold\mkern-2.5mu}
%\newcommand{\param}{\cdotold}


%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
\newcommand{\ten}[1]{\mathcal{#1}}
\newcommand{\frob}[1]{\|#1\|_2}
\newcommand{\p}[2]{\textrm{Pr}[ #1\in #2] }
\newcommand{\pe}[2]{\mathop{\textrm{Pr}}\limits_{#1}\left[#2\right] }
%\newcommand{\one}[1]{\mathds{1}[#1]}
\newcommand{\inp}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\beps}{\bm{\eps}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\RE}[3]{\E{#1}{\sup_{#2}#3}}
%\newcommand{\rc}[1]{R\left(#1\right)}

